Metric on random dynamical systems with vector-valued reproducing kernel Hilbert spaces

Development of metrics for structural data-generating mechanisms is fundamental in machine learning and the related fields. In this paper, we give a general framework to construct metrics on random nonlinear dynamical systems, defined with the Perron-Frobenius operators in vector-valued reproducing kernel Hilbert spaces (vvRKHSs). We employ vvRKHSs to design mathematically manageable metrics and also to introduce operator-valued kernels, which enables us to handle randomness in systems. Our metric provides an extension of the existing metrics for deterministic systems, and gives a specification of the kernel maximal mean discrepancy of random processes. Moreover, by considering the time-wise independence of random processes, we clarify a connection between our metric and the independence criteria with kernels such as Hilbert-Schmidt independence criteria. We empirically illustrate our metric with synthetic data, and evaluate it in the context of the independence test for random processes. We also evaluate the performance with real time seris datas via clusering tasks.

==> Metric on Random Dynamical Systems (3)/background.tex <==
\section{Background}
\label{sec:background}

In this section, we briefly review the Perron-Frobenius operators in RKHSs in Subsection~\ref{ssec:pf}, and we introduce the notion of random dynamical systems in Subsection~\ref{ssec:rds}.  In the end, we describe a  way of defining a metric for comparing two random processes with the kernel mean embeddings in Subsection~\ref{ssec:comp_rp}.

%-----
\subsection{Perron-Frobenius Opertors in RKHSs}
\label{ssec:pf}
%Here, we briefly review the RKHS (not vector-valued) and results in \cite{IFI+18}.

Let $\mathcal{X}$ be a state space and $k$ be a positive definite kernel on $\mathcal{X}$.  For any $a\in\mathcal{X}$, we denote by $k_a$ the function on $\mathcal{X}$ defined by $k_a(x)=k(a,x)$.  By Moore-Aronszajn' theorem, there exists a unique Hilbert space $\hilb_k$ composed of functions of $\mathcal{X}$ such that for any $a\in \mathcal{X}$, the function $k_a$ is contained in $\hilb_k$ and the reproducing property holds, namely, for any $f\in\hilb_k$, $\langle f, k_a\rangle_{\hilb_k}=f(a)$. The Gaussian kernel $k(x,y)=e^{-|x-y|^2}$ for $x,y\in\mathbb{R}^d$ is a typical example of the positive definite kernel.%, which is used in our empirical illustration (Section \ref{subsec: artificial}).
%Another one is the Szeg\"o kernel $k(z,w)=(1-z\overline{w})^{-1}$ for $z,w\in\mathbb{C}$ with $|z\overline{w}|\neq 1$, which appears in the context of complex analysis in pure mathematics. We will use the both kernels in Section \ref{subsec: artificial}.
%We define the feature map $\phi_k:\mathcal{X}\rightarrow\hilb_k$ by $\phi_k(x):=k_x$.

Let $\T:=\mathbb{Z}$, $\mathbb{Z}_{\ge0}$, $\mathbb{R}$, or $\mathbb{R}_{\ge0}$.  
We call a map $\varphi:\T \times \mathcal{X} \rightarrow \mathcal{X}$ a {\em dynamical system} if $\varphi(0,x)=x$ and for any $s,t\in\T$ and $x\in\mathcal{X}$ , $\varphi(s+t, x)=\varphi(s,\varphi(t, x))$.   
For $t\in\T$, we define the {\em Perron-Frobenius operator} $K_\varphi^t:\hilb_k\rightarrow\hilb_k$ by a linear operator with a dense domain, ${\rm span}\{k_x~|~x\in\mathcal{X}\}$, by
\begin{equation*}
K_\varphi^tk_x:=k_{\varphi(t,x)}.
\end{equation*}
As in the same manner as Proposition~2.1 in \cite{IFI+18}, $K_\varphi^t$ is the adjoint operator of the Koopman operator in $\hilb_k$, which is a linear operator allocating $g\in\hilb_k$ to $g(\varphi(t,\cdot))$. Note that, although the contents in \cite{IFI+18} are considered only for the discrete time case, i.e., $\T=\mathbb{Z}$ or $\mathbb{Z}_{\ge0}$, we can consider the general case $\T$. Ishikawa~et~al.~\cite{IFI+18} define a positive definite kernel by using the Perron-Frobenius operators $K_\varphi^t$ for comparing {\em deterministic} nonlinear dynamical systems, which generalizes many of the existing metrics for dynamical systems \cite{Martin00,DeCock-DeMoor02,VSV07}.

%In terms of the Perron-Frobenius operators $K_\varphi^t$, they define a positive definite kernel $\mathfrak{K}_m^T$ which measures two orbits of two dynamical systems; Here $m>0$ is a hyperparameter and $t\in\T$. Moreover, they normalize this kernel and define new kernel $A_m^T$.  Their method is quite general, thus it includes existing metrics for dynamical systems, and also handle nonlinear dynamical systems. However, their framework can treat only deterministic systems and cannot take random effect into account.

%Review of \cite{Bill99})
%-----
\subsection{Random Dynamical Systems (RDS)}
\label{ssec:rds}
%Here, we review the random dynamical systems.  
%We fix a probability space $(\Omega,  P)$.  
Let $(\Omega, P)$ be a probability space, where $\Omega$ is a measurable space, and $P$ is a probability measure. Let 
%$\T:=\mathbb{Z}$ or $\mathbb{R}$,
$\T:=\mathbb{Z}$, $\mathbb{Z}_{\ge0}$, $\mathbb{R}$, or $\mathbb{R}_{\ge0}$, 
and $\mathcal{X}$ be a state space. 
We fix a semi-group of measure preserving measurable maps $\Theta:=\{\theta_t\}_{t\in \T}$ on $\Omega$, namely, $\theta_t: \Omega\rightarrow\Omega$ such that $(\theta_t)_*P=P$, $\theta_0={\rm id}_{\Omega}$, and $\theta_s\circ\theta_t=\theta_{s+t}$ for all $s,t\in\T$. Here, $(\theta_t)_*P$ is the push-forward measure of $P$. 
%We note that, for $t\in \T$, the Koopman operator $U_{\theta_t}:L^2(\Omega)\rightarrow L^2(\Omega); f\mapsto f\circ \theta_t$ induces a bounded and isometric operator on $L^2(\Omega)$.
\begin{definition}[Random dynamical system]

Let $\mathcal{M}\subset\mathcal{X}$ be an open subset. A {\em random dynamical system} on $\Omega$ with respect to $\Theta
$ is a measurable map
\[\Phi: \T\times\Omega\times\mathcal{M}\rightarrow\mathcal{M}\]
such that $\Phi(0, \omega, x)=x$ and $\Phi(t+s, \omega, x)=\Phi\big(t,\theta_s(\omega),\Phi(s,\omega, x)\big)$ for any $x\in\mathcal{M}$. 
% We sometimes use a notation $\Phi(t, \omega): \mathcal{X}\rightarrow\mathcal{X}; x\mapsto \Phi(t, \omega ,x)$.
\end{definition}
Random dynamical systems include many kinds of stochastic processes, and typically appear as solutions of stochastic differential equations. In the case where $\Omega$ is an one point set, a random dynamical system is reduced to a deterministic one. 
\begin{example}
An auto-regressive (AR) model ``$x_{t+1}=Ax_t + v_t$'' is given as a special case of the random dynamical system as follows. Let $\T := \mathbb{Z}$, $\X:=\mathbb{R}^d$. Let $\Omega_0$ be a probability space and $v:\Omega_0\rightarrow \mathcal{X}$ be the Gaussian noise $N(0,\Sigma)$ for some $\Sigma>0$. Let $\Omega:=\Omega_0^\mathbb{Z}$.  We define $\theta_m:\Omega\rightarrow\Omega; (x_n)_n\mapsto(x_{n+m})_n$.  Put $v_m:\Omega\rightarrow\mathbb{R}^d; (x_n)\rightarrow v_m$.  Then, the function 
\begin{align*}
&\Phi(n, \omega, x) \\
&:= A(A(\cdots(Ax+v_0(\omega))+v_1(\omega))+\cdots)+v_{n-1}(\omega))
\end{align*}
is a random dynamical system with respect to $\{\theta_n\}_{n\in\T}$. Therefore, the $t$-th sample $x_t$ determined by the AR model ``$x_{t+1} = Ax_t + v_t$'' is given by $\Phi(t, \cdot, x_0)$.
\end{example}
% \begin{example}
% An auto-regressive (AR) model ``$x_{t+1}=Ax_t + v_t$'' is given as a special case of the random dynamical system as follows. Let $\T = \mathbb{Z}_{\ge0}$, $\X=\mathbb{R}^d$, $P$ be the classical Wiener measure with $\Omega = C([0, \infty))$, $W_t: \mathbb{R}_{>0}\times \Omega\rightarrow\mathbb{R}; (t,\omega)\mapsto \omega(t)$ be the Wiener process and $A\in\mathbb{R}^{d\times d}$.  Fix $\sigma>0$, and for $n\in\T$, set $v_n:=W_{(n+1)\sigma}-W_{n\sigma}$. Then $\{v_n\}$ is an i.i.d sequence of probability variables with a Gaussian distribution, and if we define $\theta_n(\omega)(t):=\omega(t+n\sigma)-\omega(t)$, then the function 
% \begin{align*}
% &\Phi(n, \omega, x) \\
% &:= A(A(\cdots(Ax+v_0(\omega))+v_1(\omega))+\cdots)+v_{n-1}(\omega))
% \end{align*}
% is a random dynamical system with respect to $\{\theta_n\}_{n\in\T}$. Therefore, the $t$-th sample $x_t$ determined by the AR model ``$x_{t+1} = Ax_t + v_t$'' is given by $\Phi(t, \cdot, x_0)$.
% \end{example}

(reason for putting the following definition)
We remark that random dynamical systems induce dynamical systems on random variables as in the following definition, which plays a main role to define Perron-Frobenius operators for RDS.
\begin{definition}
\label{DS w.r.t. RDS}
Let $\Phi$ be a random dynamical system in $\mathcal{M}$ with respect to $\Theta = \{\theta_t\}_{t\in \T}$. We define $\bm{\varphi}: \T\times M(\Omega,\mathcal{M})\rightarrow M(\Omega,\mathcal{M})$ by $\bm{\varphi}(t,X)(\omega):= \Phi\left(t,\theta_{-t}(\omega),X(\theta_{-t}(\omega))\right)$.
\end{definition}

\subsection{Comparison of Two Random Processes}
\label{ssec:comp_rp}
Here we describe a common method to define a metric for comparing two random processes \cite{Bill99}. A random dynamical system $\Phi$ in $\mathcal{M}$ gives a random processes $\{\Phi(t,\cdot,x)\}_{t\in\T}$ for each $x\in\mathcal{M}$, thus, in particular, this method provides us with a metric for random dynamical systems. 
We give its generalization in Theorem \ref{relation to KMMD} in terms of the operator theoretic method.
%It gives a positive definite kernel on random processes by means of the kernel mean embedding.


%Let $M(\T, \mathcal{X})$ be the space of measurable maps from $\T$ to $\mathcal{X}$.  
Let ${\bf X}:\Omega\rightarrow C^0(\T, \mathcal{X})$ be a stochastic process with continuous paths (for simplicity, we only consider continuous path in the case of $\T = \mathbb{R}$ or $\mathbb{R}_{>0}$). 
Let $\mathcal{L}({\bf X})$ be the law of ${\bf X}$, namely, the push-forward measure ${\bf X}_*P$ on $C^0(\T, \mathcal{X})$. The common strategy to define a metric between stochastic processes is to define the metric between the laws of the stochastic processes by the metric of a probability measure, for example, kernel maximal mean discrepancy (KMMD), Wasserstein distance, and Kullback–Leibler (KL) divergence (cf. \cite{GS02}).

Let $\kappa$ be a positive definite kernel on $C^0(\T, \mathcal{X})$. For a probability measure $\nu$, we denote by $\mu_\nu\in\hilb_\kappa$ the kernel mean embedding of $\nu$, which is given by $\int_{\Omega}\kappa_x\,d\nu(x)\in \mathcal{H}_{\kappa}$.  Then for two stochastic processes ${\bf X}$ and ${\bf Y}$, we can define the metric
\begin{equation}
\left\langle \mu_{\mathcal{L}({\bf X})}, \mu_{\mathcal{L}({\bf Y})}\right\rangle_{\mathcal{H}_{\kappa}}=\int_\Omega\kappa({\bf X}(\cdot, \omega), {\bf Y}(\cdot, \eta)) dP(\omega)dP(\eta). \label{metric for stoch process}
\end{equation}
If a positive definite kernel $k$ on $\mathcal{X}$ is given, we naturally define a positive definite kernel for $g,h\in C^0(\T, \mathcal{X})$ by $\kappa_{k,\mu}(g,h):=\int_{\mathbb{T}} k(f(t), g(t)) d\mu(t)$. 
We give  a generalization of (\ref{metric for stoch process}) in Theorem \ref{relation to KMMD} in the case where the kernel $\kappa=\kappa_{k,\mu}$ for some $k$ and $\mu$. 
%As a result, KMMD for random processes is calculated using the inner product (\ref{metric for stoch process}) as well as the case of random variables.
% For $T\in\T$, we define a positive definite kernel $k^T$ on $C^0(\T, \mathcal{X})$ by 
% \begin{align}
% 
% \end{align}

%%%--------------


==> Metric on Random Dynamical Systems (3)/conclusion.tex <==
\section{Conclusions}
\label{sec:concl}

In this paper, we developed a general framework for constructing metrics on random nonlinear dynamical systems with the Perron-Frobenius operators in vvRKHSs. vvRKHSs were employed to design mathematically manageable metrics and also to introduce $\mathcal{B}\left(L^2(\Omega)\right)$-valued kernels, which enables us to handle the randomness in systems. 
Our metric is an extension of the existing metrics for deterministic systems. Also, we generalized the Hilbert-Schmidt independence criteria to time series data. We empirically showed the effectiveness of our metric using examples of rotation dynamics with noise in the unit disk in the complex plane and clustering tasks for real time series data.  We also evaluated our metric in the context of the independence test for random processes. 

==> Metric on Random Dynamical Systems (3)/experiment.tex <==

\section{Empirical Evaluations}
\label{sec:experiment}
We first empirically illustrate how our metric behaves by using synthetic data from  rotation dynamics with noise on the unit disk in the complex plane in Subsection~\ref{subsec: artificial}, and then evaluate it in the context of the independence test for random processes in Subsection~\ref{ssec:test_eval}.  In the end, we carry out clustering task with real time series data in Subsection \ref{clustering task}.
The codes for generating the results are included in the supplementary.

\begin{figure}[t]
\begin{minipage}{0.49\hsize}
%\centering
%\hspace{-12mm}
\includegraphics[width=1\textwidth]{fig/L_sigma0_Ns1.pdf}
\subcaption{deterministic}
    \label{fig:A_sigma0}
 \end{minipage}
\begin{minipage}{0.49\hsize}
        \centering
\includegraphics[width=1\textwidth]{fig/L_sigma0_1_Ns1.pdf}
\subcaption{$\sigma=0.1, N_s=1$}
    \label{fig:A_sigma01_Ns1}
 \end{minipage}
\begin{minipage}{0.49\hsize}
        \centering
\includegraphics[width=1\textwidth]{fig/L_sigma0_1_Ns10.pdf}
\subcaption{$\sigma=0.1, N_s=10$}
    \label{fig:A_sigma01_Ns10}
 \end{minipage}
 \begin{minipage}{0.49\hsize}
        \centering
\includegraphics[width=1\textwidth]{fig/L_sigma0_5_Ns10.pdf}
\subcaption{$\sigma=0.5, N_s=10$}
    \label{fig:A_sigma05_Ns10}
 \end{minipage}
 \vspace*{-2mm}
 \caption{Discrimination results of various $(\sigma, N_s)$ pairs.
 Vertical and horizontal axes correspond to the dynamics in Figure \ref{fig:data}.
 In this experiment, the Gaussian kernel $k(z, w) := \exp{(-|z-w|^2/2)}$ for $z,w\in \mathbb{C}$ is used.
 }
 \label{fig:As}
\end{figure}

%----------
\subsection{Illustrative Example of Rotation Dynamics with Noise}
\label{subsec: artificial}
We used synthetic data from the rotation  dynamics $R_\alpha:z\mapsto\alpha z$ for $\alpha\in\mathbb{C}$ with $|\alpha|\leq 1$ with a noise $\epsilon_t$ on the unit disk $\{z\in \mathbb{C};|z|\le 1\}$ in the complex plane, where the variance of the noise is  $\sigma^2$, i.e. $\epsilon_t \sim \mathcal{N}(0, \sigma^2)$ (i.i.d.).
%\begin{align}
%z_{t+1} = \alpha z_t + \epsilon_t,
%\quad
%\epsilon_t \sim \mathcal{N}(0, \sigma^2)\text{\quad(i.i.d.)}.
%\end{align}
We prepared $3 \times 3$ combination of parameters $\alpha = |\alpha|e^{2 \pi i \theta}$ with $|\alpha| \in \{1, 0.9, 0.3 \}$ and $\theta \in \{ 1/3, 1/4, \pi/3 \}$.
The graphs in Figure \ref{fig:data} show the deterministic case and 10 independent paths for the case with $\sigma=0$ from the identical initial condition $z_0$ with $|z_0|=0.9$, where the lines of different colors show different sample paths. 
%
Then, we calculated the normalized variant of our metric defined by 
\begin{align}
&L_m^T ((\Phi_1, \bm{x}_1), (\Phi_2, \bm{x}_2))
\nonumber\\
&=
\lim_{\epsilon \to +0}
\frac{|\mathfrak{l}_m^T\left((\Phi_1, \bm{x}_1), (\Phi_2, \bm{x}_2)\right) + \epsilon |^2}
{\displaystyle\prod_{i=1}^2|\mathfrak{l}_m^T\left((\Phi_i, \bm{x}_i), (\Phi_i, \bm{x}_i)\right) + \epsilon |}
\label{eq:L}
\end{align}
with an empirical approximation of $\mathfrak{l}_m^T$ defined in \eqref{eq:estimation}. We also define $\widetilde{L}_m^T$ by replacing $\mathfrak{l}_m^T$ with $\widetilde{l}_m^T$, whose empirical estimation is given by \eqref{eq:estimation2}. %For computational costs, w
We computed $L_1^T$ and $\widetilde{L}_2^T$ here.
%
The graphs in Figure \ref{fig:As} show numerical results for some cases.
%The deterministic case (a) which was studied in \cite{IFI+18} captures similarity of $3 \times 3$ dynamics.
As can be seen in (b), if the number of samples $N_s$ 
%for approximating $\int_{\Omega^m} d \bm w$ in the definition of $\mathfrak{l}_m^T$ 
is rather small compared with the strength of the noise $\epsilon_t$, we observe that $L_1^T$ only captures rough similarity and $\widetilde{L}_2^T$ judges all dynamics are different. However, it tend to improved in (c) as the number of samples $N_s$ get larger. Also, $\widetilde{L}_2^T$ gives similar results with the deterministic case.
As for (d) where the noise level is stronger, $\widetilde{L}_2^T$ again seems to judge all dynamics are different.

%Such unwanted nature is removed if  are sufficient (c).
%It means that we can discriminate two given data of random dynamical systems in essential manner.
%Interestingly, $A_1^T$ always work roughly.
%%%%%
%\newpage
\subsection{Independence between Two Time-series Data}
\label{ssec:test_eval}
\begin{figure}[t]
\centering
\includegraphics[width=.48\textwidth]{fig/combined.pdf}
 \vspace*{-9mm}
 \caption{
 Left: Examples of two random series $X$ and $Y$ independently generated by \eqref{Xseries} and \eqref{Yseries}, and those linear combinations $X_\varphi$ and $Y_\varphi$ with $\varphi=0.35$.
 Right: plots for shift HSIC, $\hat{\bm C}_k(X_\varphi, Y_\varphi)$ and $L_m^T$ with $m=1$ and $T=20$ for $\varphi \in [0, \pi/4]$.
Each plot is normalized as max=1 min=0.
 }
 \label{fig:XYdata}
\vspace*{-2mm}
\end{figure}

We empirically evaluated the effectiveness of our metric as an independence criterion. For this purpose, we first generated $N_s=20$ pairs of complex valued time-series data with total time $T=20$ by
\begin{align}
&
x_{t+1} = 0.3 e^{\frac{2 \pi i}{3}} x_t (1- 0.01 x_t)
+ \epsilon_t^X,
\label{Xseries}
\\
&
y_{t+1} = 0.9 e^{\frac{2 \pi i}{4}} y_t (1- 0.01 y_t)
+ \epsilon_t^Y,
\label{Yseries}
\end{align}
where noises are sampled from complex normal distribution: $\epsilon_t^X, \epsilon_t^Y \sim \mathcal{CN}(0, 0.1^2)$.
We denote by $X = [x_1, x_2, \dots, x_{T=20}]$ and $Y = [y_1, y_2, \dots, y_{T=20}]$ the generated sequences. Then, we created different data pairs as
\begin{align}
&X_\varphi := X \cos \varphi + Y \sin \varphi,
\\
&Y_\varphi := - X\sin \varphi + Y\cos \varphi
.
\end{align}
By the definitions, $X_\varphi$ and $Y_\varphi$ are independent for $\varphi =0$, and correlated for $\varphi \neq 0$.
The two subplots in $\varphi=0$ column in the graphs of the left-hand side in Figure~\ref{fig:XYdata} show 10 independently generated samples for $X$ and $Y$, where the lines of different colors show different sample paths. 
On the other hand, samples of $X_{\varphi=0.35}$ and $Y_{\varphi=0.35}$ share the square shapes and seem to be correlated.

And, the graph of the right-hand side in Figure~\ref{fig:XYdata} shows the calculated $\hat{\bm C}_k(X_\varphi, Y_\varphi)$ (blue) and $L_m^T(X_\varphi, Y_\varphi)$ (red) with these sample paths. 
As a baseline, we also calculated the mean value of shift HSICs  among $20 \times 20$ paths (green) with head=10 and tail=15 \cite{CG14}. 
% \begin{align}
% &\text{Shift HSIC}(X, Y)
% =
% \Big[ p(X,Y) < 0.05 \Big],
% \notag
% \\
% &
% p(X, Y) =
% \sum_{c=\text{head}}^\text{tail}
% \frac{V(X,Y_\text{$c$-shifted}) > V(X,Y)}{\text{tail}-\text{head}},
% \notag
% \\
% &
% V(X, Y) = \frac{\text{Tr} (HK_XHL_Y)}{T^2} ,
% \left\{ \begin{array}{ll}
% (K_X)_{ts} = k(x_t, x_s) & \\
% (L_Y)_{ts} = k(y_t, y_s)  & \\
% (H)_{ts} = \delta_{ts} - \frac{1}{T}& \\
% \end{array} \right.
% ,
% \notag
% \end{align}
% where $Y_\text{$c$-shifted} = [y_c, y_{c+1}, \dots, y_T, y_1, y_2, \dots, y_{c-1}]$.
All values are normalized so that the maximum value is 1.0 and the minimum value is 0.  

As one can see, the both graphs for Shift HSIC and $\hat{\bm C}_k(X_\varphi, Y_\varphi)$ are monotone along the independence of the random processes. It is consistent to their ability to measure the independence of the systems.  In contrast,  the metric $1-L_1^T$ has a peak between 0.3 and 0.5.  It reflects that $L_m^T$ detects not the independence of the random behavior but the difference of the dynamics, which can be seen in Section \ref{subsec: artificial} as well. 


%%% ?? Results for different pairs of $(i,j)$ are given in Appendix~B in the supplementary document.

\subsection{Clustering real data}
\label{clustering task}
\begin{figure}[t]
\centering
 \includegraphics[width=0.45\textwidth]{fig/BME.pdf}\\
  \includegraphics[width=0.45\textwidth]{fig/StarLightCurves.pdf}\\
  \ % tuning hspace
  %\includegraphics[width=0.45\textwidth]{fig/Computers.pdf}
 \vspace*{-2mm}
 \caption{
 Left column: tSNE with perplexity=50 by using $1-A_1^T$.
 Right column:
 tSNE with perplexity=5 by using $1-L_1^T$.
% Results by tSNE with BME and StarLightCurves
 %and Computers 
 data.
 }
 \label{fig:BME}
\vspace*{-5mm}
\end{figure}
As an experiment using real-world data, we used UCR Archive in 2018 \cite{UCRArchive2018}.
We show results for TEST data in BME, and StarLightCurves
in Figure \ref{fig:BME}.
%The data has 3 classes, and each class consists of 50 independent paths with $T=128$.
Each data is composed of $N_c$-class pairs of $N_\text{paths}$ paths with time-length $T$.
To apply our method and compare it to the existing one, we first take $n_\text{paths} < N_\text{paths}$ paths from each class and divide it to $n_\text{pairs}$ pairs of $n_\text{sub-paths}$ paths, and calculate $(N_c\cdot n_\text{pairs}) \times (N_c\cdot n_\text{pairs})$ distance matrix using Eq.~\eqref{eq:L}, i.e. $1-L_1^T$.
We used $n_\text{paths} = 50, n_\text{pairs}=5$, i.e. $n_\text{sub-paths}=10$ in BME and StarLightCurves data.
%$n_\text{paths} = 66, n_\text{pairs}=6$, i.e. $n_\text{sub-paths}=11$ in Computer data.
We also calculated $(N_c\cdot n_\text{paths}) \times (N_c\cdot n_\text{paths})$ distance matrix using $1- A_1^T$ proposed in \cite{IFI+18} and applied tSNE \cite{Maaten08}.
To reduce the computational costs, we took skipped time series $X^\text{skipped} = [x_1, x_{s+1}, x_{2s+1}, \dots]$.
We used $s_\text{BME}=1$, ad  $s_\text{StarLightCurves} = 100$. 
%and $s_\text{Computers} = 10$.


In the left side of the Figure \ref{fig:BME}, we suppose the time series data purely comes from deterministic dynamical systems and do not take random effects into account.  On the other hand, in the right hand side, we suppose it is generated by random systems. Since our metric includes an averaging process, it could cluster BME data perfectly.  However, regarding StarLightCurves data, it seems not to be able to clearly separate two classes (red and green). This would imply the latent dynamics behind the two classes are quite similar.%, and we need another type of structural model to tell them apart.



==> Metric on Random Dynamical Systems (3)/introduction.tex <==
\section{Introduction}
%Why
%(Importance of the theory of metric for time series data generated by dynamical system. Increasing necessity of effective mathematical method to such analyze time series data with random effect <-- random dynamical system.)
%
%random dynamical systemを扱う意義の説明
%
Development of a metric for data-generating mechanisms is fundamental in machine learning and the related fields. This is because the development of an algorithm for respective learning problems according to the type of data structures in many cases is basically reduced to the design of an appropriate metric or kernel. As for the context of dynamical system, the majority of the existing metrics for dynamical systems have been developed with principal angles between some appropriate subspaces such as column subspaces of observability matrices \cite{Martin00,DeCock-DeMoor02,VSV07}. Recently, several metrics on dynamical systems are developed with transfer operators such as Koopman operators and Perron-Frobenius operators \cite{KSM19}. Mezic~et~al.~\cite{MB04,Mezic16} propose metrics of dynamical systems in the context of the ergodic theory via Koopman operators on $L^2$-spaces. Fujii~et~al.~\cite{Fujii17} developed metrics with Koopman operators as a generalization of the ones with Binet-Cauchy kernel proposed by Vishwanathan~et~al.~\cite{VSV07}. And, Ishikawa~et~al.~\cite{IFI+18} gave metrics on nonlinear dynamical systems with Perron-Frobenius operators in RKHSs, which generalize the classical ones with principal angles mentioned above.%Koopman operator ...

However, the above existing metrics are basically defined for {\em deterministic} dynamical systems. And, to the best of our knowledge, few existing literature has addressed the design of metrics for {\em random} dynamical systems or stochastic processes despite its importance for data analysis. Vishwanathan~et~al.~\cite{VSV07} mentioned their metrics for cases where systems include random noises by taking expectations over the randomness. And, Chwialkowski and Gretton ~\cite{CG14} developed non-parametric test statistics for random processes by extending the Hilbert Schmidt independence criteria.

%In machine learning, metrics for structural data is a fundamental object, and developing theories for the effective metrics is one of the main research field. 
%In this paper, we focus on analysis of time series data generated by a random dynamical system.  The random dynamical system is a natural generalization of the dynamical system in the context
%Dynamical system is a typical and important example of the data structure. 
%%deterimnistic mezic, ifi+18


%metric for stochastic process...reduces to metric for tow probability measures in a function space on $\T$. 

%How
%(random case...few (maybe, no) research exist. We generalize the method in \cite{IFI+18} to random dynamical system.  To generalize their result, we need vvRKHS.)

In this paper, we give a framework to construct metrics on {\em random} nonlinear dynamical systems, which are defined with the Perron-Frobenius operators in vector-valued reproducing kernel Hilbert spaces (vvRKHSs). Here, we employ vvRKHSs to design mathematically manageable metrics and also to introduce %$L^2(\Omega)$-valued
operator-valued kernels, which enable us to handle the randomness in systems. We first define the Perron-Frobenius operators in vvRKHSs and construct a dynamical system in a canonical way. And based on these, we define a metric on random dynamical systems as a positive definite operator-valued kernel. Our metric provides an extension of the existing metrics for deterministic systems to random ones, and gives a specification of the kernel maximal mean discrepancy of random processes. Moreover, by considering the time-wise independence of random processes, we clarify a connection between our metric and the independence criteria with kernels such as Hilbert-Schmidt independence criteria. We empirically illustrate our metric using synthetic data, and evaluate it in the context of the independence test for random processes.

The remainder of this paper is orgnized as follows. In Section~\ref{sec:background}, we first briefly review the notions necessary in this paper such as the Perron-Frobenius operators in RKHSs, and a positive definite kernel on random processes by means of the kernel mean embeddings. In Section~\ref{sec:r2d}, we construct a vvRKHS to treat random dynamical system, and define the Perron-Frobenius operators on the vvRKHSs. Then, in Section~\ref{sec:metric}, we give the definition of our metric for random dynamical systems. In Section~\ref{sec:connection}, we describe the connection of our metric to the Hilbert Schmidt independence criteria. Finally, we investigate empirically our metric using both synthetic and real data in Section~\ref{sec:experiment}, and then conclude the paper in Section~\ref{sec:concl}. All proofs are given in Appendix~A.

==> Metric on Random Dynamical Systems (3)/metric.tex <==
\section{Metrics on Random Dynamical Systems}
\label{sec:metric}

As in the previous section, we fix a bounded positive definite kernel $k$, and suppose $\mathbb{T}$ is $\mathbb{R}$ or $\mathbb{Z}$.  In this section, we construct a metric to compare two random dynamical systems.  At first, we specify the rigorous definition of the domain where our metric is defined, which we call {\em triples of random dynamical systems} with respect to $k$.  
Then we define the metric on the triples of the random dynamical systems. 
Our metric is given as a positive definite $V$-kernel for some Hilbert space (we specify $V$ later), namely it is a linear operator on $V$. 
When we evaluate this metric with a linear functional, for example the trace, it becomes a usual positive definite kernel. 
%In the end of this section, we constraint ourselves to special situations. 
Then we see our metric gives a generalization of KMMD for random processes introduced in Section \ref{ssec:comp_rp}, and define two metrics which we use in empirical computation in Section \ref{sec:experiment}.

\subsection{Definition of our metrics}
Let $\nu$ be a Borel measure on $\T$, and let $\hilb_{\rm in}$ and $\hilb_{\rm ob}$ be Hilbert spaces. 
We define triples of a random dynamical system  with respect to $k$ and $\nu$ by
$D=(L, \Phi, \I),$
%\end{equation*}
where $\Phi$ is a random dynamical system on $\mathcal{M}\subset\X$, and $\I:\hilb_{\rm in}\rightarrow\hilb_{\mathbf{k},\Phi}$ and $L:\hilb_{\mathbf{k},\Phi}\rightarrow \hilb_{\rm ob}$  such that $LK_{\Phi}^t\I$ is a Hilbert-Schmidt operator for $t\in\mathbb{T}$, and for any $v\in\hilb_{\rm in}$, the function of $t$ $||LK_{\Phi}^t\I v||_{\hilb_{\rm ob}}\in L^2(\T, \nu)$. 
We call $\I$ and $L$ an {\em initial value operator} and an {\em observable operator}, respectively.
Intuitively, the operator $L$ corresponds to an observable that gives an output at $\hilb_{\rm ob}$, and $\I$ describes an initial condition for data. We denote by
\[\mathscr{T}_k(\hilb_{\rm in}, \hilb_{\rm ob};\nu)\]
the set of the triples of random dynamical systems. 

Now, we give the definition of our metric on random dynamical systems as follows:
\begin{definition}[Metrics for RDS's]
For $i=1,2$, we fix  a triple $D_i:=(L_i, \Phi_i, \I_i)\in\mathscr{T}_k(\hilb_{\rm in}, \hilb_{\rm ob};\nu)$.
For $m\in \mathbb{N}$, $T\in \T$, we define a Hilbert-Schmidt operator by
\begin{align}
\mathscr{K}_k^{(m)}(D_1, D_2):=\bigwedge^m\int_\T\left(L_2K_{\Phi_2}^t\I_2\right)^*L_1K_{\Phi_1}^t\I_1\,d\nu(t),
\end{align}
\vspace*{-5mm}\\
and we define
\begin{align}
\mathfrak{K}_m^T(D_1, D_2):={\rm tr}\left(\mathscr{K}_k^{(m)}(D_1,D_2)\right).
\end{align}
Here, $\wedge^m$ is the $m$-th exterior product (cf.\@ Appendix~\ref{exterior product}).  
\end{definition}
Then we have the following theorem:
\begin{theorem}
\label{main thm}
The kernel $\mathscr{K}_k^{(m)}$ is a $\mathcal{B}\left(\bigwedge^m\hilb_{\rm in}\right)$-valued positive definite kernel on $\mathscr{T}_k(\hilb_{\rm in}, \hilb_{\rm ob}; \nu)$ for each $\nu$.
\end{theorem}
%We define $\mathfrak{K}_m^T$ by the positive definite kernel ${\rm tr}\left(\mathscr{K}_k^{(m)}(\cdot,\cdot)\right)$ on $\mathscr{T}_k(\hilb_{\rm in}, \hilb_{\rm ob} ;\mathbf{1}_{[0,T]}dt)$. 
We note that $\mathfrak{K}_m^T$ becomes the positive definite kernel introduced in \cite{IFI+18} in the special case where random dynamical systems are not random but deterministic. 


\subsection{Estimation of the metric}
Here we give estimaton formula (\ref{eq:estimation}) and (\ref{eq:estimation2}) below for our metric.  The proof of these formula is given in Appendix \ref{proof of estimation formula}. We use these formula to carry out the numerical experiment in Section \ref{sec:experiment}.
For $i=1,2$, let $\Phi_i$ be a random dynamical system in $\mathcal{M}_i$ and let $x_i^1,\dots,x_i^m\in\mathcal{M}_i$.  In the case of $\hilb_{\rm in}=\mathbb{C}^m$, $\hilb_{\rm ob}=\hilb_{\mathbf{k}}$, $\mathcal{I}_i((a_p)_{p=1}^m):=\sum_{p=1}^m a_p\iota(\phi(x_i^p))$ (here, $\iota$ is defined in (\ref{def of iota})),
we define 
\[\mathfrak{l}_m^T\left((\Phi_1, \bm{x}_1), (\Phi_2, \bm{x}_2)\right)
:=\mathfrak{K}_m^T((\iota^*, \Phi_1, \I_1), (\iota^*, \Phi_2, \I_2)),\]
where $\bm{x}_i:=(x_i^1,\dots,x_i^m)\in\mathcal{M}_i^m$.  Then,  we have the computation formula as follows: 
\begin{equation}
\begin{split}
&\mathfrak{l}_m^T\left((\Phi_1, \bm{x}_1), (\Phi_2, \bm{x}_2)\right)\\
&%=\int_{[0,T]^m\times\Omega^m\times\Omega^m}
=\int\label{eq:estimation}
\det\left(
k\left(\Phi_1(t_p, \omega_p, x_1^p),\,\Phi_2(t_q, \eta_q, x_2^q)\right)\right)_{p,q=1,\dots,m}
%\,d\bm{t}d\bm{\omega}d\bm{\eta},
% \begin{array}{ccc}
% \left\langle y^1_1(t_1),\,y^1_2,(t_1)\right\rangle_{\hilb_{\rm ob}}&\cdots&\left\langle y^1_1(t_1),\,y^m_2(t_m)\right\rangle_{\hilb_{\rm ob}}\\
% \vdots&\ddots&\vdots\\
% \left\langle y^m_1(t_m),\,y^1_2(t_1)\right\rangle_{\hilb_{\rm ob}}&\cdots&\left\langle y^m_1( t_m),\,y^m_2(t_m)\right\rangle_{\hilb_{\rm ob}}
% \end{array}
% &=\int_{t_1,\dots,t_m=0}^{T-1}\sum_{0<s_1<\cdots<s_
% m\le N}
% \det\left(
% \begin{array}{ccc}
% \left\langle y^{s_1}_1(t_1),\,y^{s_1}_2,(t_1)\right\rangle_{\hilb_{\rm ob}}&\cdots&\left\langle y^{s_1}_1(t_1),\,y^{s_m}_2(t_m)\right\rangle_{\hilb_{\rm ob}}\\
% \vdots&\ddots&\vdots\\
% \left\langle y^{s_m}_1(t_m),\,y^{s_1}_2(t_1)\right\rangle_{\hilb_{\rm ob}}&\cdots&\left\langle y^{s_m}_1( t_m),\,y^{s_m}_2(t_m)\right\rangle_{\hilb_{\rm ob}}
% \end{array}
% \right).
\end{split}
\end{equation}
where the variable $(t_1,\dots,t_m, \omega_1,\dots,\omega_m, \eta_1,\dots,\eta_j)$ in the integral runs over $[0,T]^m\times\Omega^m\times\Omega^m$.
In particular, our metric is a generalization of KMMD for an integral type kernel, which is given through the following theorem: 
\begin{theorem}\label{relation to KMMD}
Let 
\[\kappa_T(g,h):=\int_0^Tk(g(t), h(t))d\nu(t)\]
be an integral type kernel on $C^0(\T, \mathcal{X})$, then we have
\begin{align*}
&\mathfrak{l}_1^T\left((\Phi_1, \bm{x}_1), (\Phi_2, \bm{x}_2)\right)= 
\left\langle \mu_{\mathcal{L}\left(\Phi_1(\cdot,\cdot,x_1^1)\right)},\,  \mu_{\mathcal{L}\left(\Phi_2(\cdot,\cdot,x_2^1)\right)}\right\rangle_{\hilb_{\kappa_T}}.
\end{align*}
\end{theorem}
This theorem implies for general $m$, the metric $\mathfrak{l}_m^T$ is a reasonable generalization for two random dynamical systems in the context of KMMD. However,  for higher $m$, 
the formula (\ref{eq:estimation}) needs a heavy calculation. To improve the drawback of (\ref{eq:estimation}), we construct another metric as follows: Let $\hilb_{\rm ob}:=\hilb_{\mathbf{k}}$, and define 
\begin{equation*}
\widetilde{\mathfrak{l}}_m^T((\Phi_1, \bm{x}_1), (\Phi_2, \bm{x}_2))\\
:=\mathfrak{K}_m^T\left(({\rm id}_{\hilb_{\mathbf{k}}}, \Phi_1, \I_1), ({\rm id}_{\hilb_{\mathbf{k}}}, \Phi_2, \I_2)\right).
\end{equation*}
Then we have the following formula:
\begin{align}
&\widetilde{\mathfrak{l}}_m^T\left((\Phi_1, \bm{x}_1), (\Phi_2, \bm{x}_2)\right)\nonumber\\
&=\int
%_{[0,T]^m\times\Omega^m}
\det\left(
k\left(\Phi_1(t_p, \omega_p, x_1^p),\,\Phi_2(t_q, \omega_q, x_2^q)\right)\right)_{p,q=1,\dots,m}
%\,d\bm{t}dP(\bm{\omega})
.\label{eq:estimation2}
\end{align}
where the variable $(t_1,\dots,t_m, \omega_1,\dots,\omega_m)$ in the integral runs over $[0,T]^m\times\Omega^m$.

==> Metric on Random Dynamical Systems (3)/relation_hsic.tex <==
\section{Connection to Hilbert-Schmidt Independence Criteria}
\label{sec:connection}
In this section, we argue a relation between our operator-valued positive definite kernel and Hilbert-Schmidt independence criteria (HSIC). We first define a independence criterion for random dynamical systems based on the above contexts, and then give its estimator. Our independence criterion measures a pairwise independence of random dynamical systems. Although our metric is constructed in the context of the dynamical system, it can also be used to extract the information about the independence of two systems. This is a main reason to introduce the vvRKHS above. 



\subsection{A brief review of Hilbert-Schmidts independence criterion}

%As in the previous sections, let $(\Omega,P)$ be a probability space.
We first briefly review HSIC \cite{GBSS05}.  Let $X, Y:\Omega\rightarrow\mathcal{X}$ be two random variables. And, let $k$ be a positive definite kernel on $\mathcal{X}$. Here, we assume that $k$ is characteristic, namely, the kernel mean embedding is injective \cite{SFL10}. Also, we define the {\em cross covariance operator} $C_k(X,Y):\hilb_k\rightarrow\hilb_k$ by
\[C_k(X,Y):=\int_{\Omega}\left(\rule{0pt}{9pt}k_{X(\omega)}-\mu_X\right)\otimes\left(\rule{0pt}{9pt}k_{Y(\omega)}-\mu_Y\right)\,dP(\omega),\]
where $\mu_X, \mu_Y\in\hilb_k$ are the kernel mean embeddings of the lows $X_*P$ of $X$ and $Y_*P$ of $Y$, respectively. We regard any element of $\hilb_k\otimes\hilb_k$ as a bounded linear operator on $\hilb_k$, namely, for any $v\otimes w\in\hilb_k\otimes\hilb_k$, we define $v\otimes w\in\B(\hilb_k)$ by $(v\otimes w)(x):= \langle w, x\rangle v$. 
We note that via the identification, $\hilb_k\otimes\hilb_k$ is equal to the space of Hilbert-Schmidt operators, in particular, the cross-covariance operator $C_k(X,Y)$ is also a Hilbert-Schmidt operator.  
Straightforward computations show that 
\[C_k(X,Y)=\mu_{[XY]}-\mu_X\otimes\mu_Y,\]
where $[XY]:\Omega\rightarrow\mathcal{X}\times\mathcal{X}; \omega\rightarrow (X(\omega), Y(\omega))$. 
The characteristic property of $k$ shows that $C_k(X,Y)=0$ if and only if $X$ and $Y$ are independent. The HSIC is defined to be 
${\rm HSIC}_k(X, Y):=||C_k(X,Y)||_{\rm HS}^{2}:={\rm tr}(C_k(X,Y)^*C_k(X,Y)),$ which is the Hilbert-Schmidt norm of $C_k(X,Y)$. The value ${\rm HSIC}_k(X, Y)$ can be estimated via the evaluation of kernel functions over samples (see \cite[Lemma 1]{GBSS05}). 


\subsection{HSIC for random dynamical systems}
Let us consider the independence of random dynamical systems in our context.  For $i=1,2$, let $\Phi_i$ be a random dynamical system on $\mathcal{X}$. 
We fix $x_1,x_2\in\mathcal{X}$, and let $\mathbf{X}:=\{X_t\}_{t\in\T}=\{\Phi_1(t,\cdot, x_1)\}_{t\in\T}$, $\mathbf{Y}:=\{Y_t\}_{t\in\T}=\{\Phi_2(t,\cdot, x_2)\}_{t\in\T}$.  We set $\hilb_{\rm in}:= L^2(\Omega)$ and $\hilb_{\rm ob}:=\hilb_k$.
%We impose $K_{\bm{\phi}_i, L^2(\Omega)}^t$ exists.
We define $\I_{x_i}(h):=\mathbf{k}_{x_i}\left(h-\int_\Omega h\right)$. 
Set $D_i:=(\iota_k^*, \Phi_i, \I_{x
_i})\in\mathscr{T}_k(\hilb_{\rm in},\hilb_{\rm ob};\nu_i)$. We define the independent criteria for random dynamical systems by
\begin{align}
&\mathbf{C}_k((\Phi_1,x_1,\nu_1), (\Phi_2, x_2, \nu_2))\nonumber\\
&:={\rm tr}\left(\mathscr{K}^{(1)}_k(D_1,D_1)\mathscr{K}^{(1)}_k(D_2,D_2)\right).
\end{align}
% Let $\alpha>0$.  We define the following function:
% \begin{align}
% \mathscr{D}_k^\alpha(\varepsilon; X,Y):=\varepsilon^{-2-\alpha}\log\frac{\Delta_{k^{\oplus2}}(\varepsilon; [XY],[XY])}{\Delta_k(\varepsilon; X,X)\Delta_k(\varepsilon; Y,Y)}
% \mathscr{D}_k^\alpha(\varepsilon; X,Y):=\varepsilon^{-2-\alpha}\left(\rule{0pt}{9pt}\Delta_{k^{\oplus2}}(\varepsilon; [XY],[XY])-\Delta_k(\varepsilon; X,X)\Delta_k(\varepsilon; Y,Y)\right)
%\mathscr{D}_k^\alpha(z; X,Y)
%:=\Delta_{k^{\oplus2}}(z; [XY],[XY])-\Delta_k(z; X,X)\Delta_k(z; Y,Y)
% \end{align}
% where we define $k^{\oplus 2}((x,y),(z,w)):=k(x,z)+k(y,w)$ on $\mathcal{X}\times\mathcal{X}$.  

% In fact, $\mathcal{D}_k^\alpha(\varepsilon;\cdot,\cdot)$ gives an independent criteria, more precisely, we have the following theorem.
Then, we have the following relation:
\begin{theorem}
\label{relation to HSIC}
We have
\begin{align*}
    &\mathbf{C}_k((\Phi_1,x_1,\nu_1), (\Phi_2, x_2, \nu_2))\\
    &=\int_\T\int_\T C_k(X_s, Y_t)d\nu_1(s)d\nu_2(t).
\end{align*}
% For any $s,t\in\T$, we have
% \[\mathbf{C}_k((\Phi _1,x_1,\delta_s), (\Phi_2, x_2, \delta_t))=C_k(X_s, Y_t).\]
% Here $\delta_t$, $\delta_s$ are Dirac's delta with mass at $t$.
\end{theorem}
% This theorem means our independent criteria recovers time-wise independent criteria of HSIC.


\begin{figure}[t]
\begin{minipage}{0.49\hsize}
        \centering
\includegraphics[width=1\textwidth]{fig/sigma_0.pdf}
\subcaption{deterministic}
    \label{fig:data_sigma0}
 \end{minipage}
 %%
\begin{minipage}{0.49\hsize}
        \centering
\includegraphics[width=1\textwidth]{fig/sigma_0_1.pdf}
\subcaption{$\sigma=0.1, N_s=10$}
    \label{fig:data_sigma02}
 \end{minipage}
 \vspace*{-2mm}
 \caption{Orbits of rotation dynamics by (a):just multiplying $\alpha= |\alpha|e^{2\pi i \theta}$ with same initial values, (b): multiplying $\alpha$ and perturb it by Gaussian noise with variance $\sigma^2$.
 }
 \label{fig:data}
 %%%
\end{figure}


Next we consider the estimation of $\mathbf{C}_k$.
%%%%%%多分いらない%%%%%%%%
% At first we give the following lemmas:
% \begin{lemma}
% Let $\Phi$ be a random dynamical system on $\mathcal{M}$, and fix $x\in\mathcal{M}$ and finite Borel measure $\nu$ on $\T$. Put $Z_t(\omega):=\Phi(t,\omega, x)$.  Let $\ell_{k,D}(t;\cdot,\cdot)$ be the positive definite kernel on $\Omega$ defined by
% \begin{align}
% \ell_{k,D}(t;x,y):=&k(x,y)-\int_{\Omega}k(x,Z_t(\omega))dP(\omega)\nonumber- \int_{\Omega}k(Z_t(\omega), y)dP(\omega) \\
% &+ \int_{\Omega^2}k(Z_t(\omega),Z_{t}(\omega'))dP(\bm{\omega}),
% \end{align}
% where $\bm{\omega}=(\omega,\omega')$ is defined in the same way.
% Then $\mathscr{K}_k^{(1)}(D,D,\nu):L^2(\Omega)\rightarrow L^2(\Omega)$ is the operator induced by the kernel $\int_\T\ell_{k,D}(t;Z_t(\cdot),Z_t(\cdot))d\nu(t)$, namely, $\mathscr{K}_k^{(1)}(D,D;\nu) h (\omega)=\int_\Omega\int_\T h(\eta)\ell_{k,D}(t;Z_t(\eta),Z_t(\omega))dP(\eta)d\nu(t)$.
% %Moreover, for any $m>0$, we have
% % \begin{align}{\rm tr}\mathscr{K}_k^{(m)}(D, D; \delta_t)=\frac{1}{m
% % !}\int_{\Omega^m}\int_{\T^m}\det
% % \left(\ell_{k,D,\nu}(Z_{t_i}(\omega_i),Z_{t_j}(\omega_j))\right)_{i,j=1,\dots,m}
% % d\nu(\bm{t})dP(\bm{\omega}).
% % \end{align}
% % where $\nu(\bm{t})=d\nu(t_1)\dots d\nu(t_m)$ ,and  $\bm{\omega}$ is defined in the same way.
% \end{lemma}
% \begin{lemma}
% \label{trace of wedge}
% Let $T_l:L^2(\Omega)\rightarrow L^2(\Omega)$ be linear operator induced by the kernel $l\in L^2(\Omega^2)$. Then we have ${\rm tr}\bigwedge^m T_l
% =(m!)^{-1}\int_{\Omega^m}\det\left(\ell(\omega_i,\omega_j)\right)_{i,j=1,\dots,m}$.
% \end{lemma}
% \begin{lemma}
% \label{a formula for HS op}
% Let $V$ be a Hilbert space, and let $A,B:V\to V$ be Hilbert-Schmidt operators.  Then we have ${\rm tr}AB = {\rm tr}A\cdot {\rm tr}B+{\rm tr}\bigwedge^2A + {\rm tr}\bigwedge^2B - {\rm tr}\bigwedge^2(A+B).$
% \end{lemma}
Let $\{X^{(1)}_t\}_{t\in\T}$, $\dots$, $\{X^{(n)}_t\}_{t\in\T}$ and $\{Y^{(1)}_t\}_{t\in\T}$,$\dots$,$\{Y^{(n)}_t\}_{t\in\T}$ be independent $n$ sample passes for $\mathbf{X}$ and $\mathbf{Y}$, respectively. 
Set $\mathbf{Z}:=\mathbf{X}$ or $\mathbf{Y}$, $Z_t^{(p)}:=X_t^{(p)}$ or $ Y_t^{(p)}$, $D:=D_i$, and $\nu:=\nu_i$. We define 
\begin{align}
\widehat{k}_{D}^{(n)}(t;x,y)\nonumber&:=k(x,y)-\frac{1}{n}\sum_{p=1}^nk(x,Z_{t}^{(p)})\nonumber\\
&\hspace{-30pt}- \frac{1}{n}\sum_{i=p}^nk(Z_{t}^{(p)}, y) + \frac{1}{n^2}\sum_{p,q=1}^nk(Z_{t}^{(p)},Z_{t}^{(q)}).
\end{align}
Let $\widehat{G}_{k,D}^{(n)}(t) := \left(\widehat{k}_{D}^{(n)}(Z_t^{(p)}, Z_t^{(q)})\right)_{p,q=1,\dots,n}$ be a matrix of size $n$. By Theorem \ref{relation to HSIC}, and Theorem 1 in \cite{GBSS05}, we have an estimator of $\mathbf{C}_k((\Phi_1, x_1, \nu_1), (\Phi_2, x_2, \nu_2))$  as 
\begin{align}
\label{estimator}
&\widehat{\mathbf{C}}_k((\Phi_1, x_1, \nu_1), (\Phi_2, x_2, \nu_2))\nonumber\\
&:=\frac{1}{(n-1)^2\#S_1\#S_2}\sum_{(s,t)\in S_1\times S_2}{\rm tr}\left(G_{k,D_1}^{(n)}(s)G_{k,D_2}^{(n)}(t)\right),
\end{align}
where $S_1$ and $S_2$ are finite samples according to $\nu_1$ and $\nu_2$, respectively.
% Let
% \begin{align*}
% \widehat{\tau}_{\mathbf{Z},m}^{(n)}&:=\frac{1}{m!n^m}\sum_{i_1,\dots,i_m=1}^n\det\left(\frac{1}{\#S}\sum_{t\in S}\widehat{\ell}_{k,D}^{(n)}(t;Z_{t}^{(p)}, Z_{t}^{(q)})\right)_{p,q=1,\dots,m},\\
% \widehat{\rho}_m^{(n)}&:=\frac{1}{m!n^m}\sum_{i_1,\dots,i_m=1}^n\det\left(\frac{1}{\#S_1}\sum_{t\in S_1}\widehat{\ell}_{k,D_1}^{(n)}(t;X_{t}^{(p)}, X_{t}^{(q)})+\frac{1}{\#S_1}\sum_{t\in S_2}\widehat{\ell}_{k,D_2}^{(n)}(t;Y_{t}^{(p)}, Y_{t}^{(q)})\right)_{p,q=1,\dots,m},
% \end{align*}
% where $S, S_1$, and $S_2\subset\T$ are a finite sample according to $\nu$, $\nu_1$, and $\nu_2$, respectively. Then by Lemma \ref{trace of wedge} and Lemma \ref{a formula for HS op}, we have the estimation of $\mathbf{C}_k$:
% \[\widehat{\mathbf{C}}_k^{(n)}((\Phi_1,x_1,\delta_s), (\Phi_2, x_2, \delta_t)):=\widehat{\tau}_{\mathbf{X},1}^{(n)}\widehat{\tau}_{\mathbf{Y},m}^{(n)}+\widehat{\tau}_{\mathbf{X},2}^{(n)}+\widehat{\tau}_{\mathbf{Y},1}^{(n)}-\widehat{\rho}_{2}^{(n)}.\]
% The convergence as $n\rightarrow\infty$ follows from the large number low.
% \begin{remark}
% Let $G_n^{\mathbf{Z}}:=\left(k(Z_t^{(i)}, Z_t^{(j)})\right)_{i,j=1,\dots,n}$, and let $\mathbf{1}_n$ be the matrix whose components are all 1. Put $H_n:=I_n-n^{-1}\mathbf{1}_n$  Then $\widehat{\tau}_{\mathbf{Z},m}^{(n)}={\rm tr}H_nG_nH_n$
% \end{remark}

% We remark that in \cite{BJ02}, Bach and Jordan define the kernel generalized variance (KGV) for investigation of independent component analysis. More precisely, the definition of the KGV is given by
% \[KGV(X,Y):=\frac{\det\left(\kappa + C_{k^{\oplus2}}([XY],[XY])\right)}{\det\left(\kappa + C_k(X,X)\right)\det\left(\kappa + C_k(Y,Y)\right)},\]
% where $\kappa$ is suitable small positive number.
% Then we have the following formula
% \begin{proposition}
% \[\exp\left(\kappa^{-2-\alpha}\mathscr{D}_k^\alpha(\kappa^{-1}; X, Y)\right)=KGV(X, Y)\]
% \end{proposition}


% Let us consider independence of random dynamical systems in our context.  For $i=1,2$, let $\Phi_i$ be a random dynamical system on $\mathcal{X}$ with respect to $\Theta_i$. 
% We define the random dynamical system on $\mathcal{X}^2$ by $\Phi_3:=(\Phi_1, \Phi_2)$. 
% We fix $x_1,x_2\in\mathcal{X}$, and let $x_3:=(x_1, x_2)\in\mathcal{X}^2$.
% %and $t\in\T$
% , and let $X_t(\omega)=\Phi_1(t,\omega, x_1)$, $Y_t(\omega)=\Phi_2(t,\omega, x_2)$, and $[X_tY_t](\omega)=(X_t(\omega),Y_t(\omega))$. We set $\hilb_{\rm in}:= L^2(\Omega)$ and $\hilb_{\rm ob}:=\hilb_k$. We define $\I_i(h):=\left(h-\int_\Omega h\right)\iota_k(k_{x_i})$,  ($i=1,2$), $\I_3(h)=\iota_{k^{\oplus2}}(k^{\oplus2}_{x_3}$, and $L_i:=\iota_k^*$. Put $D_i:=(L_i, \Phi_i, \I_i)$. For $z\in\mathbb{C}$, we define
% \begin{align}
% \Delta_k(z; X, Y)&:=\det\left(\rule{0pt}{9pt}1-z \mathscr{K}_k^{(1)}(D_1, D_2; \delta_t)\right)\nonumber\\
% &:=\sum_{m=0}^\infty(-1)^m{\rm tr}\mathscr{K}_k^{(m)}(D_1, D_2; \delta_t)z^m.
% \end{align}
% We note that $\Delta(z; X,Y)$ is an entire function on $\mathbb{C}$, which follows Proposition \ref{} in Appendix \ref{appendix for wedge}).   In this situation, we have the following formulas:
% \begin{proposition}
% For $i=1,2$, the triple $D_i$ is as above. Let $\ell_{k,X,Y}$ be the positive definite kernel defined by
% \begin{align}
% \ell_{k,X,Y}(x,y):=&k(x,y)-\int_{\Omega}k(x,Y(\omega))dP(\omega)\nonumber\\
% &- \int_{\Omega}k(X(\omega), y)dP(\omega) + \int_{\Omega}\int_{\Omega}k(X(\omega),Y(\omega'))dP(\omega) dP(\omega).
% \end{align}
% Then $\mathscr{K}_k^{(1)}(D_1,D_2,\delta_t):L^2(\Omega)\rightarrow L^2(\Omega)$ is the operator induced by the kernel $\ell_{k,X,Y}(X,Y)$, namely, $\mathscr{K}_k^{(1)}(D_1, D_2;\delta_t) h (\omega)=\int_\Omega h(\eta)\ell_{k,X,Y}(\eta,\omega)dP(\eta)$.
% Moreover, we have
% \begin{align}{\rm tr}\mathscr{K}_k^{(m)}(D_1, D_2; \delta_t)=\frac{1}{m
% !}\int_{\Omega}\dots\int_{\Omega}\det
% \left(\ell_{k,X,Y}(X(\omega_i),Y(\omega_j))\right)_{i,j=1,\dots,m}
% dP(\omega_1)\dots dP(\omega_m).
% \end{align}
% \end{proposition}
% Let $\alpha>0$.  We define the following function:
% \begin{align}
% \mathscr{D}_k^\alpha(\varepsilon; X,Y):=\varepsilon^{-2-\alpha}\log\frac{\Delta_{k^{\oplus2}}(\varepsilon; [XY],[XY])}{\Delta_k(\varepsilon; X,X)\Delta_k(\varepsilon; Y,Y)}
% % \mathscr{D}_k^\alpha(\varepsilon; X,Y):=\varepsilon^{-2-\alpha}\left(\rule{0pt}{9pt}\Delta_{k^{\oplus2}}(\varepsilon; [XY],[XY])-\Delta_k(\varepsilon; X,X)\Delta_k(\varepsilon; Y,Y)\right)
% %\mathscr{D}_k^\alpha(z; X,Y)
% %:=\Delta_{k^{\oplus2}}(z; [XY],[XY])-\Delta_k(z; X,X)\Delta_k(z; Y,Y)
% \end{align}
% where we define $k^{\oplus 2}((x,y),(z,w)):=k(x,z)+k(y,w)$ on $\mathcal{X}\times\mathcal{X}$.  

% In fact, $\mathcal{D}_k^\alpha(\varepsilon;\cdot,\cdot)$ gives an independent criteria, more precisely, we have the following theorem.
% \begin{theorem}
% \label{relation to HSIC}
% % Let $\mathscr{D}_k^\alpha(z; X,Y):=\sum_{n=0}^\infty c_k(n;X,Y)z^n$ be the taylor expansion at 0. Then we have the following formula:
% % \begin{align*}
% % c_k(0; X,Y)&=c_k(1;X,Y)=0,\\
% % c_k(2; X,Y)&={\rm HSIC}_k(X,Y).
% % \end{align*}
% \begin{align*}
% \mathscr{D}_k^\alpha(\varepsilon; X, Y)&=\varepsilon^{-\alpha}{\rm HSIC}_k(X, Y)+O(\varepsilon^{1-\alpha}).
% \end{align*}
% In particular, we have
% \begin{align*}
% \lim_{\varepsilon\rightarrow0}\mathscr{D}_k^{\alpha}(\varepsilon
% ; X, Y)=
% \begin{cases}
% 0 & \text{ if $X$ and $Y$ are independent},\\
% {\rm HSIC}_k(X,Y) & \text{ if $X$ and $Y$ are dependent and $\alpha = 0$},\\
% \infty & \text{ if $X$ and $Y$ are dependent and $\alpha>0$}.
% \end{cases}
% \end{align*}
% \end{theorem}
% In empirical computation, we take a small $\epsilon>0$, thus, this theorem implies that hyperparameter $\alpha$ gives $\mathscr{D}_k^\alpha$ sensitivity for the independence of two random variables. The larger we take $\alpha>0$, the more sensitive $\mathscr{D}_k^\alpha$ becomes.

% Let $\{X_1,\dots,X_n\}$ and $\{Y_1\dots, Y_n)\}$ be independent samples for $X$ and $Y$, respectively. We define estimated version of $\ell_{k,X,Y}$, ${\rm tr}\mathcal{K}_1(D_1,D_2,\delta_t)$, and $\widehat{\Delta}_k(z;X,Y)$ by
% % , and $\widehat{D}_k(z; X,Y)$
% \begin{align}
% \widehat{\ell}_{k,X,Y}^{(n)}(x,y)&:=k(x,y)-\frac{1}{n}\sum_{i=1}^nk(x,Y_i)\nonumber
% \\
% &\hspace{20pt}- \frac{1}{n}\sum_{i=1}^nk(X_i, y) + \frac{1}{n^2}\sum_{i,j=1}^nk(X_i,Y_j),
% \\
% \widehat{t}_{k,m}^{(n)}(X,Y)&:=\frac{1}{m!n^m}\sum_{i_1,\dots,i_m=1}^n\det\left(\widehat{\ell}_{k,X,Y}^{(n)}(X_{i_p}, Y_{i_q})\right)_{p,q=1,\dots,m},
% \\
% \widehat{\Delta}_{k}^{(n)}(z; X,Y)&:=1-\widehat{t}_1^{(n)}(X,Y)z+\widehat{t}_2^{(n)}(X,Y)z^2,\label{emperical delta}
% % \\
% % \widehat{D}_k^{(n)}(z; X,Y)&:=\log\frac{1-\widehat{t}_1^{(n)}([XY],[XY])z+\widehat{t}_2^{(n)}([XY],[XY])z^2}{(1-\widehat{t}_1^{(n)}(X,X)z+\widehat{t}_2^{(n)}(X,X)z^2)(1-\widehat{t}_1^{(n)}(Y,Y)z+\widehat{t}_2^{(n)}(Y,Y)z^2)}
% \end{align}
% respectively.  As we are only interested in at most the second order of $\mathscr{D}_k(z;X,Y)$ for $z$ with small $|z|$, We cut off the third and more orders in (\ref{emperical delta}).

% We remark that in \cite{BJ02}, Bach and Jordan define the kernel generalized variance (KGV) for investigation of independent component analysis. More precisely, the definition of the KGV is given by
% \[KGV(X,Y):=\frac{\det\left(\kappa + C_{k^{\oplus2}}([XY],[XY])\right)}{\det\left(\kappa + C_k(X,X)\right)\det\left(\kappa + C_k(Y,Y)\right)},\]
% where $\kappa$ is suitable small positive number.
% Then we have the following formula
% \begin{proposition}
% \[\exp\left(\kappa^{-2-\alpha}\mathscr{D}_k^\alpha(\kappa^{-1}; X, Y)\right)=KGV(X, Y)\]
% \end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Let $\theta: \Omega\rightarrow\Omega$ be a measurable map satisfying $P= \theta_*P$.  We define $\Gamma_\theta( \hilb)$, the quotient of the space of measurable maps $\bm{\gamma}=(\alpha, \gamma): \Omega \rightarrow\Omega \times \hilb$ such that $\alpha =\theta$ and $||\gamma(\cdot)||_{\hilb}\in L^2(P)$ divided by the space of functions $\bm{\delta}$ satisfying $\bm{\delta}(\omega) = (\theta(\omega),0)$ $P$-a.e..
% %For any $v\in\hilb$, we define $c(\theta,v)\in\Gamma(\hilb)$ by $c(\theta,v)(\omega):=(\theta(\omega), v)$.
% We note that $\Gamma_\theta( \hilb)$ naturally becomes a Hilbert space with inner product defined by $\left\langle  \bm{\gamma}_1, \bm{\gamma}_2\rangle :=\int_{\Omega}\langle \gamma_1(\omega), \gamma_2(\omega)\rangle_{\hilb}\,d\theta_*P(\omega)$ for $\bm{\gamma}_i=(\theta, \gamma_i)$ $(i=1,2)$.
% For another $\theta':\Omega\rightarrow\Omega$, we define the pull-back $c_{\theta'}: \Gamma_{\theta}( \hilb)\rightarrow \Gamma_{\theta\theta'}( \hilb)$ by $c_{\theta'}(\bm{\gamma})(\omega):=\bm{\gamma}(\theta'(\omega))$. 

% \begin{proposition}
% There exists a unique Hilbert space $\hilb_{k_\Phi}$ with morphisms  $\{i_t:\Gamma_{\theta_t}(\hilb)\}_{t\in \T}\rightarrow\hilb_{k_\Phi}$ such that $i_{t+s}=c_{\theta_t}i_s$ and for any morphisms $\left\{j_t:\Gamma_{\theta_t}(\hilb)\rightarrow \hilb'\right\}_{t\in\T}$ with $j_{t+s}\circ c_{\theta_s}=j_t$, there uniquely exists a map $j:\hilb_{k_\Phi} \rightarrow \hilb'$ such that $j_t = j\circ i_t$.
% \end{proposition}

% We remark that $\hilb$ is regarded as a closed subspace of $\hilb_{k_\Phi}$ via the map $\iota_k: \hilb\rightarrow \hilb_{k_\Phi}; v\mapsto i_0(\theta_0, v)$. Moreover, the adjoint $\iota_k^*$ is an integral operator defined by $\iota_k^*\big(i_t(\theta_t, \gamma)\big)=\int_\Omega\gamma(\omega)dP(\omega)$.

% Then we define a Hilbert space
% % \[\bm{\Gamma}_\Theta(\Omega,\hilb)=\lim_{\underset{t}{\longrightarrow}}\Gamma_{\theta_t}(\Omega,\hilb)\]
% \begin{align*}
% \bm{\Gamma}_\Theta(\Omega, \hilb)
% &:=\lim_{\underset{t}{\longrightarrow}}\Gamma_{\theta_t}(\Omega,\hilb)=\bigoplus_{t\in\T}\Gamma_{\theta_t}(\Omega,\hilb)\big\slash
% \left\{(\bm{\gamma}_{\theta_s})_{s\in\T}
% % \in\bigoplus_{t\in\T}\Gamma_{\theta_t}(\Omega,\hilb)
% ~\big|~
% c_{\theta_t}(\bm{\gamma}_{\theta_s})-c_{\theta_s}(\bm{\gamma}_{\theta_s})\text{ for }s,t\in \T
% %\cdot\displaystyle\sum_{\theta\text{:$P$-inv.}}||\gamma_\theta||^2<\infty
% \right\}
% \end{align*}

%We denote by $\bm{\Gamma}(\Omega,\hilb):=\bigsqcup_{\theta}\Gamma_\theta(\Omega, \hilb)$.  

% \begin{definition}
% Let $\Phi$ be a random dynamical system with respect to $\Theta$. 
% For $t\in \T$, we define the Perron-Frobenius operator $K_\Phi^t: \hilb_{k_\Phi}\rightarrow\hilb_{k_\Phi}$ by a linear operator with domain ${\rm span}\left\{i_t\left(\theta_t, \phi(X)\right)~\big|~X:\Omega\rightarrow\X\text{: measurable}\right\}$ 
% satisfying
% \[K_\Phi^ti_s(\theta_s, \phi(X)):=\left(\theta_{t+s}, \phi(\Phi(t,\theta_{t}, X))\right).
% % \begin{cases}
% % (\theta_{u}, \phi(\Phi(t,\theta_u, X_u))
% % &\text{ if }u=s+t,\\[2pt]
% % (\theta_u, 0)&\text{otherwise.}
% % \end{cases}
% \]
% \end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
%\section{Estimation from empirical data}
% ...


==> Metric on Random Dynamical Systems (3)/vvrkhs.tex <==
\section{Perron-Frobenius operators for random dynamical systems}
\label{sec:r2d}

In this section, we define a Perron-Frobenius operator for random dynamical systems, % endowed with a positive definite kernel,% \cite{}, and we define a Perron-Frobenius operator on RKHS in this setting.
 which is a natural generalization of the operator defined in
 \cite{IFI+18} in Subsection~\ref{ssec: PF op on vvRKHS}. vvRKHSs are employed to introduce operator-valued positive definite kernels,  which enables us to incorporate the effects of random variables.  
 %Then, we introduce the notion of random dynamical systems, and construct a dynamical system on random variables in a canonical way in Subsection~\ref{ssec:rds}. 
 These notions %a little complicated, but it 
are generalizations of the corresponding deterministic case (namely, the case where $\Omega$ is an one point set).  %, and gives a nice framework to analyze the operators for random dynamical systems.
For simplicity, in this section, we assume $\mathbb{T}=\mathbb{R}$ or $\mathbb{Z}$.  %For the general situation, see Appendix \ref{}.

%-----
\subsection{A brief review of vector-valued RKHSs}
\label{ssec: vvRKHS}
Let $\bm{\mathcal{X}}$ be a set and $V$ be a Hilbert space. We denote by $\mathcal{B}(V)$ the space of bounded linear operators in $V$. We define a $\mathcal{B}(V)$-valued positive definite kernel ${\bf k}$ as a map ${\bf k}:\mathcal{X}\times\mathcal{X}\rightarrow \mathcal{B}(V)$ satisfying the following two conditions: (1) for any $x,y\in \mathcal{X}$, ${\bf k}(x,y)={\bf k}(y,x)^*$, and (2) for any $r\in \mathbb{N}$, $v_1,\dots,v_r\in V$, and $x_1,\dots,x_r\in \mathcal{X}$, $\sum_{i,j=1}^r\left\langle {\bf k}(x_i,x_j)v_i, v_j\right\rangle_V\ge0$. We note that ``$\mathcal{B}(V)$-valued positive definite kernel'' is equivalent to ``$V$-valued kernel of positive type'' in \cite{CVT06}. We define a linear map ${\bf k}_y: V\rightarrow V^{\mathcal{X}}$ by $({\bf k}_yv)(x)={\bf k}(y, x)v$ for $v\in V$. We note that $\mathbb{C}$-valued positive definite kernel is the equivalent notion to the positive definite kernel in Section \ref{ssec:pf}.
%We define the feature map $\phi_{{\bf k}}: \mathcal{X}\rightarrow \mathcal{B}(V)^{\mathcal{X}}$ by $\left(\phi_{{\bf k}}(x)\right)(y)={\bf k}(x,y)$.

For any $\mathcal{B}(V)$-valued positive definite kernel $k$, it is well known that there uniquely exists a Hilbert space $\hilb_{{\bf k}}$ in $V^{\mathcal{X}}$ such that for any $x\in \mathcal{X}$ and $v\in V$, ${\bf k}_xv\in \hilb_{{\bf k}}$, and for any $h\in\hilb_{{\bf k}}$, $\langle h, {\bf k}_ xv\rangle_{\hilb_{{\bf k}}}=\langle h(x),v\rangle_V$ (see Proposition 2.3 in \cite{CVT06}). We call $\hilb_{{\bf k}}$ the vector-valued reproducing kernel Hilbert space associated with ${\bf k}$ or the $V$-valued reproducing kernel Hilbert space associated with ${\bf k}$. 

We note that we can canonically construct RKHSs from the vvRKHS as in the following proposition:
\begin{proposition}
\label{k from vvRKHS}
For any $v\in V$, the kernel $k_v(x,y):=\langle v, {\bf k}(x,y)v\rangle_V$ is a ($\mathbb{C}$-valued) positive definite kernel. Moreover, the RKHS $\mathcal{H}_{k_v}$ associated with $k_v$ is isomorphic to the closed subspace of $\mathcal{H}_{{\bf k}}$ defined by the closure of the ${\rm span}\{{\bf k}_xv : x\in\mathcal{X}\}$. 
\end{proposition}

%We note that in the case where ${\bf k}(x,y)$ is a trace class operator for each $x,y\in\mathcal{X}$, ${\rm tr}({\bf k}(x,y))$ is a positive definite kernel since the trace of ${\bf k}(x,y)$ is given by ${\rm tr}({\bf k}(x,y)) := \sum_{i\in I}\langle {\bf k}(x,y)e_i,e_i\rangle_V$, where $\{e_i\}_{i\in I}$ is an orthonormal basis of $V$.

\subsection{vvRKHS on random variables}
\label{ssec: vvRKHS on random variables}
Here, we gives vvRKHS for random variables by specifyng vvRKHS described above, 
%give a key example of vvRKHS,
which plays a central role in the following parts of this paper.

Let $k$ be a bounded and continuous ($\mathbb{C}$-valued) positive definite kernel on a topological space $\mathcal{X}$, and let $(\Omega, P)$ be a probability space with the probability measure $P$.  We denote by $M(\Omega, \mathcal{X})$ the space of $\mathcal{X}$-valued random variables. Now, we define a vvRKHS on $M(\Omega, \mathcal{X})$ in terms of the given kernel $k$.

\begin{definition} 
We define the $\mathcal{B}\left(L^2(\Omega)\right)$-valued positive definite kernel $\mathbf{k}$ on $M(\Omega, \mathcal{X})$ by
%\[\left(\mathbf{k}(\gamma, \gamma')h\right)(\omega) := U_{\gamma_\Omega'}^*k(\gamma_\X(\omega),\gamma_\X'(\omega))U_{\gamma_\Omega}h(\omega),\]
\[\left(\mathbf{k}(X, Y)f\right)(\omega) := k(X(\omega),Y(\omega))f(\omega),\]
where 
%we define$m_{k(\gamma_\X,\gamma_\X')}f(\omega)=k(\gamma(\omega),\gamma'(\omega))f(\omega)$, and 
$X, Y\in M(\Omega, \mathcal{X})$.
\end{definition}
We note that $\mathbf{k}(X,Y)$  induces a bounded linear operator such that $||\mathbf{k}(X,Y)||:=\sup_{\omega\in\Omega}|k(X(\omega),Y(\omega))|$. We may define a natural positive definite kernel for random variables as the expectation of $k(X,Y)$, but, we can mathematically deduce this kernel in our framework: Let $\mathbf{1}\in L^2(\Omega)$ be a constant function valued 1.  We see that we can construct the positive definite kernel $k_{\mathbf{1}}(X,Y):=\mathbb{E}_P[k(X, Y)]$ by Proposition \ref{k from vvRKHS}.
 



%-----


\subsection{Perron-Frobenius Operators for RDS}
\label{ssec: PF op on vvRKHS}
In this subsection, we construct Perron-Frobenius operators for random dynamical systems.  Random dynamical systems include random effects in addition to the structure of dynamical systems.  To this end, we utilize the vvRKHS in Section \ref{ssec: vvRKHS on random variables}, and construct linear operators on the vvRKHS by means of the dynamical systems defined in Definition \ref{DS w.r.t. RDS}. 

%Here, we construct a dynamical system and an $L^2(\Omega)$-valued RKHS on a set of random variables in terms of a given random dynamical system. This dynamical system enables us to study random dynamical systems in terms of theories of deterministic dynamical systems. We also need the $L^2(\Omega)$-valued  RKHS to scrutinize the random effect in the systems via Perron-Frobenius operators and the kernel method. Moreover, we finally describe our Perron-Frobenius operators generalize the existing operators for random processes.

%We fix a {\em bounded} positive definite kernel $k$ on $\mathcal{X}$ and let $\hilb_k$ be the corresponding RKHS. Let $M(\Omega,\mathcal{M})$ be the set of measurable maps.  For each random dynamical system $\Phi$, we construct a dynamical system in $M(\Omega,\mathcal{M})$ in a canonical way, which is same as the push-forward of the skew product \cite[1.1.8]{Arno98} of the random dynamical system. 


%Let $\M_{\mathcal{M}}$ be the set of measurable maps $\gamma = (\gamma_\Omega, \gamma_\mathcal{M}): \Omega\rightarrow\Omega\times\mathcal{M}$ such that the Koopman operator $U_{\gamma_\Omega}$ induces a bounded linear operator on $L^2(\Omega)$.  For each random dynamical system $\Phi$, we construct a dynamical system in $\M_{\mathcal{M}}$ in a canonical way, which is same as the push-forward of the skew product \cite[1.1.8]{Arno98} of the random dynamical system. 

First, let $\mathcal{X}$ be a topological space and let ${\bf k}$ be the $\mathcal{B}(L^2(\Omega))$-valued positive definite kernel on $\mathcal{X}$ as in Proposition \ref{ssec: vvRKHS on random variables}.   For any subspace $\mathcal{M}\subset\mathcal{X}$, and random dynamical system $\Phi$ in $\mathcal{M}$, we define
a closed subspace $\hilb_{{\bf k}, \Phi}\subset\hilb_{{\bf k}}$ as the closure of ${\rm span}\left\{{\bf k}_Xh~\big|~X=\Phi(t,\cdot,x), x\in\mathcal{M}, t\in\mathbb{T}, h\in L^2(\Omega)\right\}$.  
\begin{definition}[Perron-Frobenius operators for RDS]
For $t\in\T$, we define the $t$-th {\em Perron-Frobenius operator} for RDS $\Phi$ by the linear operator $K_{\Phi}^t:\hilb_{{\bf k}, \Phi}\rightarrow\hilb_{{\bf k},\Phi}$ with the domain ${\rm span}\left\{{\bf k}_Xh~\big|~X=\Phi(t,\cdot,x), x\in\mathcal{M}, t\in\mathbb{T}, h\in L^2(\Omega)\right\}$ such that $K_{\Phi}^t{\bf k}_Xh={\bf k}_{\bm{\varphi}(t,X)}h$, where $\bm{\varphi}$ is the dynamical system defined in Definition \ref{DS w.r.t. RDS}.
\end{definition}

We give some connections between our operators and other existing operators:
% We note that $K_{\varphi, W}^t$ does not always exist, and its existence rather depends on the choice of the subspace $W\subset V$. 



% Let $M(\Omega, \mathcal{X})$ be the set of measurable maps, and let $\theta_t^*$ be the pull-back maps on $M(\Omega, \mathcal{X})$, i.e., $\theta_t^*(\gamma)=\gamma\circ\theta_t$.   Now, we show that there exists a canonical deterministic dynamical system associated with the random dynamical system $\Phi$ as follows:

% \begin{proposition}
% \label{prop: canonical dynamical system}
% There exists a ${\bf M}_\Theta$ and the family of maps $\{i_t:M(\Omega, \mathcal{X})\rightarrow {\bf M}_\Theta\}_{t\in \T}$ such that $i_{t}=i_{t+s}\circ \theta_s^*$ for $s,t\in\T$, and satisfies the following universality: for any set $\mathcal{Y}$ and a family of maps  $\{j_t:M(\Omega, \mathcal{X})\rightarrow \mathcal{Y}\}_{t\in \T}$ with  $j_{t}=j_{t+s}\circ \theta_s^*$ for $s,t\in\T$, there uniquely exists a map $j:{\bf M}_\Theta\rightarrow \mathcal{Y}$ such that $j_s=j\circ i_s$ for all $s\in \T$.
% \end{proposition}
% \begin{proof}
% See Appendix ...
% \end{proof}
% We remark that in the case of $\T=\mathbb{Z}$ or $\mathbb{R}$, the space ${\bf M}_\Theta$ is just the space $M(\Omega, \mathcal{X})$ and $i_s:=\theta_{-s}^*$. 

% We construct the dynamical system associated with the random dynamical system as follows: Fix $t\in\T$, then for any $s\in\T$, we define $j_s:M(\Omega, \mathcal{X})\rightarrow {\bf M}_\Theta$ by $j_s(\gamma):=i_{t+s}\left(\Phi(t, \theta_s, \gamma)\right)$, here $\Phi(t, \theta_s, \gamma)\in M(\Omega, \mathcal{X})$ is defined by $\Phi(t, \theta_s, \gamma)(\omega):=\Phi(t, \theta_s(\omega), \gamma(\omega))$ for $\omega\in\Omega$. Since $j_{s+t}\circ\theta_t=j_t$, by the universal property of ${\bf M}_\Omega$ in Proposition \ref{prop: canonical dynamical system}, there exists $\bm{\varphi}_t: {\bf M}_\Omega\rightarrow{\bf M}_\Omega$.  Now, we define the canonical dynamical system $\bm{\varphi}:\T\times{\bf M}_\Omega\rightarrow{\bf M}_\Omega$ by $\bm{\varphi}(t, \gamma):=\bm{\varphi}_t(\gamma)$. The map $\bm{\varphi}$ is actually a dynamical system, namely,
% \begin{proposition}
% For $s,t\in\T$, we have $\bm{\varphi}(s+t, \gamma)=\bm{\varphi}(s, \bm{\varphi}(t, \gamma))$.
% \end{proposition}
% \begin{proof}
% See Appendix ...
% \end{proof}



\paragraph{Connection to Perron-Frobenius operators for random processes}
We show that our operator is a generalization of the Koopman operator defined in \cite{CZMM19}, namely, the Perron-Frobenius operator $K_{\Phi}^t$ completely recovers the classical transfer operator in Proposition \ref{random Koopman} below.
Let 
\begin{align}
\iota:\hilb_k\rightarrow\hilb_{\mathbf{k}} \label{def of iota}
\end{align}
be %$\iota_k(h)(\gamma):=U_{\gamma_{\Omega}}^*(h\circ\gamma_\X)$,
$\iota(h)(X):=(h\circ X)$,
and regard $\hilb_k$ as a closed subspace of $\hilb_{\mathbf{k}}$. 
Accurately, at first, we define $\iota(k_x):=\mathbf{k}_x\mathbf{1}$, and then show it induces the well-defined linear map from $\mathcal{H}_k$ to $\mathcal{H}_{\mathbf{k}}$.  
Note that for $g\in \hilb_{\mathbf{k}}$, the adjoint of $\iota$ is defined to be $(\iota^*g)(x)=\mathbb{E}_P[g(x)]$. Here we regard $x\in\mathcal{M}$ as a constant function on $\Omega$, and $g(x)\in L^2(\Omega)$. 
\begin{proposition}\label{random Koopman}
For any $x\in\mathcal{X}$, we have
\[\iota^*K_{\Phi}^{t}\iota(k_x)=\int_\Omega k_{\Phi(t,\omega,x)}dP(\omega).\]
\end{proposition}
% Although the following proposition is obvious by the definition, it is worth remarking thaat $\{K_\Phi^t\}_{t\in\T}$ has the semi-group property:
% \begin{proposition}
% We have $K^0_\Phi = {\rm id}$, and for $s,t\in\T$, $K_\Phi^{s+t}=K_\Phi^{s}\circ K_\Phi^t$.
% \end{proposition}

\paragraph{Connection to Koopman operators on vvRKHS}
Here, we show the relation between existing operators in vvRKHS and our operator.  In the case where a dynamical system is deterministic ($\Omega$ is an one-point set), discrete-time ($\T=\mathbb{Z}$ or $\mathbb{Z}_{>0}$). Then $K_{\Phi}^1$ is the same one defined in \cite{IFI+18}.  
Let $\mathcal{M}=\mathcal{X}$. In \cite{FK19}, they define the Koopman operator for a discrete-time dynamical system by the linear operator $g\mapsto g\circ f$ for $g\in \hilb_{\mathbf{k}}$, where we put $f:=\varphi(1,\cdot)$. As stated in the following proposition, their operator is given as the adjoint of the Perron-Frobenius operator:
\begin{proposition}\label{adjoint of Koopman}
We have $(K_{\varphi}^1)^*=\mathcal{K}_{{\bf k}}$, where $\mathcal{K}_{{\bf k}}$ is the Koopman operator defined in \cite{FK19} (we give a rigorous definition of the Koopman operator in the proof of this proposition).
\end{proposition}
